Is the Pope Catholic? Yes, the Pope is Catholic. Generative Evaluation of Non-Literal Intent Resolution in LLMs

Humans often express their communicative intents indirectly or non-literally, which requires their interlocutors -- human or AI -- to understand beyond the literal meaning of words. While most existing work has focused on discriminative evaluations, we present a new approach to generatively evaluate large language models' (LLMs') intention understanding by examining their responses to non-literal utterances. Ideally, an LLM should respond in line with the true intention of a non-literal utterance, not its literal interpretation. Our findings show that LLMs struggle to generate pragmatically relevant responses to non-literal language, achieving only 50-55% accuracy on average. While explicitly providing oracle intentions significantly improves performance (e.g., 75% for Mistral-Instruct), this still indicates challenges in leveraging given intentions to produce appropriate responses. Using chain-of-thought to make models spell out intentions yields much smaller gains (60% for Mistral-Instruct). These findings suggest that LLMs are not yet effective pragmatic interlocutors, highlighting the need for better approaches for modeling intentions and utilizing them for pragmatic generation.

==> sections/0-abstract-v1.tex <==
Conversational agents based on Large language models (LLMs) must understand pragmatics to effectively communicate with humans, who often speak indirectly. Existing work, mostly through multiple-choice tests, tend to oversimplify pragmatic understanding and overestimate LLMs' capabilities.  In our work, we propose a new evaluation framework which instead examines the ability of LLMs to infer latent intentions and generate pragmatic responses. 
%This generative evaluation provides a more precise evaluation that aligns closely with real-world LLM applications. 
LLMs should ideally respond to non-literal utterances in line with the user's true intent rather than a literal misinterpretation. Our findings show that LLMs struggle to generate pragmatic responses to non-literal language. While chain-of-thought prompting minimally improves their performance, providing explicit cues about user's true intended meaning results in increased improvements. These findings highlight the importance of explicit intention modeling and mental states representations in LLMs.

==> sections/4-jen_data.tex <==
\section{Pragmatic Understanding Dataset}
\label{sec:data}
To measure pragmatic understanding in LLMs, we adopt evaluation materials from \citet{hu2022fine}. \citet{hu2022fine} frame each item as a multiple choice question, with the answers representing different interpretations of the speaker's intentions. In Figure \ref{fig:figure_1}, ``\akhila{intention 1}'' and ``\akhila{intention 2}'' are two ways of interpreting what ``\akhila{speaker character}'' intended to convey.  

\par To test pragmatic response generation, we reformat this data to: 
\begin{enumerate}
    \itemsep0em
    \item \textbf{Context $C$}: Short story involving 2 or more characters 
    \item \textbf{Non-literal Utterance $U_1^N$}: Speaker generates an utterance using non-literal language 
    \item \textbf{True Intention $I_T$}: The actual intended meaning  of the speaker 
    \item \textbf{Incorrect Literal Intention $I_L$}: An incorrect literal interpretation of the speaker's intention
\end{enumerate}
% might have to elaborate in the appendix 
We consider four non-literal phenomenon from \citet{hu2022fine}: Indirect Speech, Irony, Maxims of conversation and Metaphors.\footnote{\maarten{add a note that there were others but we didn't include them (e.g., Deceit is too non-cooperative)}}
\par \textbf{Indirect Speech.} In indirect speech, speakers often implicate more than what is explicitly stated, commonly to make requests. For example, saying ``Can you reach the salt?'' may function not only as a question but also as a request for someone to pass the salt. 
%\daniel{I'm not sure that indirect requests are typically called performatives?}
\par \textbf{Irony.} In this setting, speakers uses irony to convey the opposite semantic content of their utterances.  Irony is not explicitly defined within context $C$, but the context itself may include information about characters' emotional states.
\par \textbf{Maxims of conversation.} In this task, speakers deliberately violate one of Grice's conversational maxims, which are principles governing effective communication, such as quantity, quality, relevance, and manner \cite{searle}. 
%\daniel{if space, make this more self-contained even if people don't know Grice.}
\par \textbf{Metaphor.} In this task, the speaker uses metaphors to draw comparisions between entities in a non-literal sense. 
% \daniel{if we have space, it would help to give an example of each of these. Or, minimally, we should give an example of $C$, $U_1^N$, etc. for one particular utterances.} % this is addressed now!

==> sections/5-direct_intention_understanding.tex <==
\section{Discriminative Intention Understanding}
%\maarten{Revisit this when we've written the intro, cause a lot of this could be said in the intro and just briefly stated again here (in 1-2 sentences), focusing on the need for direct measurement due to discrepancies between MC and generation \cite{hu2023prompting,yejinParadoxPaper}.}
To highlight the importance of our proposed generative approach for evaluating pragmatic understanding, which focuses on assessing implicit intention understanding in responses (i.e turn 2), we contrast this with commonly used discriminative evaluations in prior work \cite{hu2022fine, grice, ..} that focus on contrastively detecting true intention of speaker utterances (i.e turn 1). 
%In contrast, prior work \cite{hu2022fine, grice, ..} has often evaluated LLMs' pragmatic understanding abilities in a discriminative multiple-choice setup. To contrast the pragmatic abilities of LLMs in discriminative vs generative settings, we follow the methodology used in \citet{hu2022fine} and measure probabilities of each answer option (e.g., ``1'', ``2'').  


\subsection{Method and Evaluation}
We adopt the methodology used in \citet{hu2022fine}, which uses a multiple-choice setup and measures probabilities of each answer option. They compute the probability of answer options -- true intention $I_T$ and literal misinterpretation $I_L$ -- given the context $C$, the speaker's non-literal utterance $U_1^N$, and task instructions. We measure accuracy as assigning the highest probability to the correct answer token (e.g., ``1'', ``2''). Refer to Appendix \ref{app:disc_jenn_prompt} for prompt template used. 


%We compute the log likelihood of each candidate intention ($I_T$ and $I_L$) under the given context $C$ and speaker's non-literal utterance usage $U_1^N$ i.e we measure $P(I | C, U_1^N)$ for each $I = \{ I_T, I_L\}$. We measure accuracy as ranking the true intention $I_T$ higher than $I_L$. 
%To effectively measure language models' ability to infer the intended meaning of a speaker's non-literal utterance $U_1^N$ under context $C$, we propose computing direct probabilities. This involves evaluating language models' performance using generative evaluation rather than a multiple-choice discriminative setting. We gauge intention understanding by computing $P(I | C, U_1^N)$ where $I = \{ I_T, I_L\}$. Essentially, we measure the log probability of each candidate intention or interpretation under the given the context and non-literal utterance usage.

%\akhila{look at adding confidence calibration}
%\daniel{can we justify this better, maybe by saying that we find that it works better? It's unclear whether we're making a design choice here or introducing an improvement on past work.} 

%\subsection{Noisy Channel Measurement}
%P(U | C, I) * P(I|C) $\propto$ P(I | C, U) \\
%Drawing inspiration from noisy channel models in machine translation \cite{} and their extension to other tasks \cite{}, we want to measure intention understanding via channel models. We use Bayes' rule to reparameterize $(I | C, U_1^N)$ as $\frac{P(U_1^N | C, I) * P (I | C)}{P(U_1^N | C)}$. As we are usually interested in the $argmax_{I_i \in I} \frac{P(U_1^N | C, I_i) * P (I_i | C)}{P(U_1^N | C)}$, it is sufficient to model $P(U_1^N | C, I_i) * P (I_i | C)$. This decomposes into 2 components:  $P(U_1 | C, I_i)$ measures how probable is utterance $U_1^N$ under a given context $C$ and intention $I_i$ and $P (I_i | C)$ represents a prior measurement of an intention $I_i$ under context $C$. 
%\akhila{talk about why this is a cool measurement: how does first part how when utterance is non-literal? second part shows how much explicit intention modeling based on the context plays a role in pragmatic understanding}
%\daniel{nice!}


\subsection{Experiments and Results}
\label{ssec:explicit_experiments}
\quad \textbf{Models.} \quad We compare the same models as in Section \label{ssec:response:models}\footnote{We cannot evaluate against models behind APIs like GPT-4 due to lack of access to input-token probabilities.}.

%\textbf{Evaluation.} \quad We measure accuracy by comparing the log probability of the true intention $I_T$ with the log probability of the alternative incorrect intention $I_L$, assigning higher accuracy to the intention with the higher log probability. We compare the performance of models under this setup with metalinguistic measurement using multiple-choice as used in \citet{hu2022fine}. \akhila{to-do rerun comparing with Jen -- rerun with just 2 intentions}

\textbf{Results.} \quad Similar findings reported by \citet{hu2022fine}, we observe that larger models, specifically LLama2-70b-chat, outperforms others across all phenomenon. In the case of Indirect Speech, smaller models around 7b size (except Mistral) find the generative setting easier than the discriminative setting. Mistral, however, finds the contrastive discriminative setting significantly easier. 

In the discriminative setting, we consistently see that models are able to detect true intention when conversational norms (maxims) are violated, but struggle with appropriately responding based on this inferred intent.Further, LLama2 models are more successful in recognizing the true intention when interpreting metaphorical language in a contrastive setting.

We see that trends do not remain consistent across different models and phenomena, and, on average, models struggle more in the generative setting.  This underscores the importance of evaluating model performance in \textit{both} discriminative and generative settings to obtain a better understanding of LLMs' pragmatic understanding.

%\akhila{I have no idea how to tie it together with these results -- but enough differences to point out -- need help}




%\par As models predominantly outperform random chance only on the Indirect Speech task, we measure Pearson correlation of models' performance between this discriminative setting and our proposed generative setting. We get a $\rho = 0.25$ for Indirect Speech, which implies that generative and discriminative settings for pragmatic intention understanding are distinct –- thus improved performance in commonly used discriminative settings does not necessarily lead to enhanced pragmatic response generation. 
%\daniel{this kind of leaves me (and potentially reviewers) wondering what the point of this setting is. Maybe both the explicit and implicit settings are just noisy? it would help if we could say how this compares to prior work -- did they also find that models were typically around random chance?}


%As shown in Figure \ref{fig:intention_accuracy_exp1}, LLMs perform best on Indirect Speech, but they struggle with understanding violations of conversational maxims (Maxim), ironic utterances that convey the direct opposite of the speaker's belief (Irony), and \textbf{especially} with the figurative language used in metaphors (Metaphor).  While larger models like LLama2-70b and more efficient models like Mistral perform the best, we did not observe any significant differences based on model size or architecture for this discriminative pragmatic understanding setting. 


%find that direct probability measurements are a tighter evaluation than the multiple-choice setup using \citet{hu2022fine}, with models performing worse on our evaluation setup. \maarten{This suggests that... [something about how MC over-estimated the model's pragmatic understanding abilities]} 
%\maarten{Add a sentence or two on model size perhaps if there are any interesting results?}

%However, the relative trends on performance on each task is similar. We and \citet{hu2022fine} both find that models find Indirect Speech task easier. Models struggle most with understanding disobedience of conversational maxims (Maxims) and understanding ironic utterances conveying the direct opposite of the speaker's belief (Irony). One stark difference is the performance on Metaphors. We find that metaphors, requiring more global knowledge beyond what is conveyed \maarten{incomplete sentence, wouldn't say too much more for space reasons.}

%\akhila{ \\
%- worse than Jen!
%- similar trends in both direct and noisy \\
%- llama2-70b and mistral are better \\ 
%-deceits, indirect speech are easier \\ 
%- irony, metaphor and maxims are harder tasks \\
%-in noisy channel, we see the importance of prior P(I|C) in task of understanding non-literal utterances. }
%\daniel{if both direct and noisy work equally well, are there other things that noisy channel adds (e.g. can we do some nice analysis on the importance of the prior?) If not, we could just choose one (e.g. direct, since that's more common in past work?), and then focus mostly on the implicit intention understanding}




